A unified framework for correlation mining in ultra-high dimension

Many applications benefit from theory relevant to the identification of variables having large correlations or partial correlations in high dimension. Recently there has been progress in the ultra-high dimensional setting when the sample size $n$ is fixed and the dimension $p$ tends to infinity. Despite these advances, the correlation screening framework suffers from practical, methodological and theoretical deficiencies. For instance, previous correlation screening theory requires that the population covariance matrix be sparse and block diagonal. This block sparsity assumption is however restrictive in practical applications. As a second example, correlation and partial correlation screening requires the estimation of dependence measures, which can be computationally prohibitive. In this paper, we propose a unifying approach to correlation and partial correlation mining that is not restricted to block diagonal correlation structure, thus yielding a methodology that is suitable for modern applications. By making connections to random geometric graphs, the number of highly correlated or partial correlated variables are shown to have compound Poisson finite-sample characterizations, which hold for both the finite $p$ case and when $p$ tends to infinity. The unifying framework also demonstrates a duality between correlation and partial correlation screening with theoretical and practical consequences.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

==> sections/redudant_contributions.tex <==
\section{Comparisons and Contributions}

Contributions:
\begin{enumerate}
	\item 
	This paper contains all theoretical results from "Large scale correlation screening" and "Hub screening in partial correlation graph". This paper additionally characterize the full distribution converges in distribution to a compound Poisson in a unified framework as in Theorem \ref{cor:Poissonlimit} when $p$ goes to infinity and Theorem \ref{thm:Poissonultrahigh} for finite but large $p$. 
	
	\item This paper take a geometric perspective, and make connections to random geometric graph, see Subsection \ref{sec:rangeo}. With this view, it is more natural to see the number of subgraphs isomorphic to a star graph is approximately compound Poisson (cf. Subsection \ref{sec:closenessnumedge}). The geometric results (Lemmas \ref{prop:rangeo}, \ref{prop:rangeolimit} and \ref{lem:randgeogra}) are also of independent interest. With the 3 geometric Lemmas we go from the finite p compound Poisson approximation (cf. Theorem \ref{thm:Poissonultrahigh}) to a limiting Poisson approximation (cf. Theorem \ref{cor:Poissonlimit}) and further show for reasonably large $n$ or $\delta$, the limiting compound Poisson is approximately a Poisson (cf. Section \ref{sec:limitingcompoundPoisson}).
	
	\item This paper relaxes the sparsity assumption from block-$\tau$ sparsity to $(\tau,\kappa)$ sparsity for empirical partial correlation graph, which allows more correlation between variables. 
\end{enumerate}	

\noindent 
Comparisons:
\begin{enumerate}	
	\item 
	This paper correct the result $\P(\bar{N}_\delta >0 )$ for $\bar{N}_\delta\in \{N_{E_\delta}^{(k)},N_{\breve{V}_\delta}^{(k)},N_{V_\delta}^{(k)}: k\in \{\Rma,\Pma\}  \}$ in "Hub screening in partial correlation graph" since it should converges to the probability of same event for a compound Poisson. This paper also correct a convergence rate in "Large scale correlation screening" (not essential).
	
	\item Comparing to the two previous papers, theorems in the current paper are strengthened by weakening the assumptions made in the previous papers. On one hand, all the assumptions are on the model parameter $\Sigmama$ but not on some intermediate quantity show up in the proof. On the other hand, we relax some of the assumptions in the previous paper, like "the (conditional) joint density of $\Uma$-score are bounded"
	
	\begin{comment}
	\item (too detail. just for our own knowledge) This paper simplifies the assumptions. See the following tables for comparison of assumptions between our current paper and "Large scale correlation screening" in empirical correlation graph. As discussed, the matrix-elliptically contoured distribution assumption is to guarantee the fact "if $\Sigmama_{ij}=0$ then $\uve_i$ and $\uve_j$ are independent", which is used in "Large scale correlation screening" but not well justified. So the matrix elliptically contour assumption on data matrix is not really an additional assumption, and with this, we manage to drop many assumptions that is difficult to verify, as shown in the table. One additional assumption in this paper is "$\mu_{n,2\delta+2}(\Sigmama)$ bounded by a constant independent of $p$", and this assumption can be easily verify by Lemma \ref{lem:sufass}.  One goal for this paper is to only make assumption that can be easily verify and avoid making assumptions on intermediate quantities, joint density of $\Uma$-score for instance, and only make assumption on the initial parameters and model. Much efforts are put to achieve this goal.
	
	The comparison between our current paper and "Hub screening paper in Partial Correlation Graph" for empirical partial correlation graph is similar and thus is omitted. 
	\\ 
	\begin{tabular}{|c|c|c|}\hline	  
		empirical correlation graph &  large correlation paper  & our current paper \\ \hline
		matrix elliptically contour & \xmark & \cmark  \\ \hline
		row-$\kappa$ sparse & \cmark & \cmark \\ \hline
		joint density of $\Uma$-scores multiplying by $|S^{n-2}|^p$ are bounded & \cmark & \xmark \\ \hline
		derivative of joint density multiplying by $|S^{n-2}|^p$ are bounded & \cmark & \xmark \\ \hline
		conditional density of $\Uma$-score multiplying by $|S^{n-2}|^p$ are bounded & \cmark & \xmark \\ \hline
		$\mu_{n,2\delta+2}(\Sigmama)$ bounded by a constant independent of $p$  & \xmark & \cmark \\ \hline
	\end{tabular}
	\end{comment}
	
	\item Our model is random pseudo geometric graph on unit sphere. It's related to random geometric graph. In Penrose' book \cite{penrose2003random} in 2003 independent vertices is assumed, while our model allow some possible correlations between vertices (more comparisons are in Subsection \ref{sec:rangeo}). In the Example after Corollary 3.6 in \cite{penrose2003random}, the author makes comments on the number of vertices of degree $\delta$ is asymptotically a compound Poisson (but without characterizing the parameters of the limiting compound Poisson). Here in our paper we give a full characterization of the limiting compound Poisson distribution.
	
\end{enumerate}


==> sections/redudant_introduction.tex <==
\section{Old versions abstracts}\YW{by Prof. Rajaratnam}

\begin{abstract}
	
{\bf Proposed abstract}
An important problem in large scale inference is the identification of variables that have large correlation or partial correlation with at least one other variable. Recent work in correlation screening has yielded breakthroughs in the ultra-high dimensional setting when the sample size $n$ is fixed and the dimension $p \rightarrow \infty$ (see \cite{hero2012hub}). Despite these advances, the correlation screening framework suffers from some serious practical, methodological and theoretical deficiencies. For instance, theoretical safeguards for partial correlation screening requires that the population covariance matrix be block diagonal. This block sparsity assumption is however highly restrictive in numerous practical applications. As a second example, results for correlation and partial correlation screening framework requires the estimation of dependence measures or functionals, which can be highly prohibitive computationally, rendering the framework impractical and unappealing in the very setting it is designed for. In this paper, we propose a unifying approach to correlation and partial correlation screening which specifically allows for dependence in the underlying true correlation structure, thus yielding a methodology that is suitable for modern applications. Theoretical expressions for false discovery probabilities are obtained for finite $p$. The approach also obviates the need to estimate dependence measures rendering the framework readily scalable. The unifying framework also demonstrates an important duality between correlation and partial correlation screening with important theoretical and practical consequences.	
	
\textbf{Contributions of this paper}:
\begin{enumerate}
	\item Obtain the results on $(\tau,\kappa)$ sparsity, see Proposition \ref{thm:meannumdis}, \ref{thm:var} and Theorem \ref{falposratest}. $(\tau,\kappa)$ sparsity is a broader assumption than block sparsity assumption, see Section \ref{sec:taukappaspa} for detailed comparison.
	\item have two sections (section \ref{sec:distancepreserving} and section 7) discussing why results for partial correlation screening is the same as correlation screening. Specifically, Proposition \ref{uyrelation} in Section  \ref{sec:distancepreserving} shows the distance between columns of $\Yma$-score are preserved to associated columns of $\Uma$-score by coefficients depending on the condition number of a random matrix. Then Lemma \ref{proeig} in Section \ref{ranmatunisph} establishes for those type random matrix, the condition number is close to 1 with high probability.
	\item have a new result (Theorem \ref{thm:var}) on the variance of number of discovery, which can be used to establish a non-trivial lower bound for discovery rate (Corollary \ref{cor:discoveryrate}) through 2nd moment method
	\item 
	The approximations don't depend on the quantity $J$. The original results for correlation screening (Proposition 1 in \cite{hero2011large}) establish the results with dependence on $J$. In \cite{hero2012hub}, for both correlation and partial correlation screening, Proposition 1 and 2 establish results depending on $J$, then Proposition 3 establish that $J$ is close to 1 under block sparse condition. The current paper is similar the structure of \cite{hero2012hub}, but we just combine the fact that $J$ is close to 1 into the bounds so that the approximation is simpler, and is under the $(\tau,\kappa)$ sparsity. But in the proof, in fact, we actually establish results on $J$, and the fact that $J$ is close to $1$. So in appendix right before the proof instead of the main body, comes the definition of $J$.
	\item The approximations are obtained for finite $p$. For example, Theorem \ref{falposratest} \ref{item:fprcor} establishes the approximation for discovery rate in correlation screening case for all $p$. While Theorem \ref{falposratest} \ref{item:fprpar} establish approximations for discovery rate in partial correlation screening case provided \eqref{eqn:plar2} holds. \eqref{eqn:plar2} is quantitative way of saying $p$ is large enough, as explained after Proposition \ref{thm:meannumdis}.
\end{enumerate}	
	
\end{abstract}


\section{Introduction\YW{old versions by Prof. Rajaratnam}}
In this paper we consider the problem of screening $\nn$ independent and identically distributed $p$-variate samples for variables that have high correlation or high partial correlation with at least one other variable in the ultra-high dimensional regime when the sample size $\nn \leq C_0\ln p$.\footnote{Here $C_0$ is some universal constant satisfying $C_0\geq 1$. A ``universal constant" or ``absolute constant", is a constant that does not depend on any model parameter.} In the screening framework one applies a threshold to  sample correlation matrix or the sample partial correlation matrix to detect variables with at least one significant correlation. This threshold aims to separate signal from noise. Correlation and partial correlation screening in ultra-high dimensions has become increasingly important in many modern applications as the per-sample cost of collecting high dimensional data is much more costly than per-variable cost. For example, in biomedical settings the cost of high throughput technology, like oligonucleotide gene microchips and RNAseq assays is decreasing, while the cost of biological samples isn't decreasing at the same rate \cite{hero201615}. In such situations $p$ is much larger than $\nn$.

The ultra-high dimensional regime when $\nn\leq C_0\ln p$ is very challenging since the number of samples is insufficient to apply many (if not most) reliable statistical methods. For example, one way to do the screening is firstly estimate the population covariance matrix, from which one estimates the inverse covariance, which is a proper estimation to the partial correlation matrix. However, to get a reliable estimate for general covariance matrix, the number of samples $\nn$ must be at least $O(p)$ as shown in Section 5.4.3. in \cite{vershynin2012introduction}. Even if the covariance matrix has special structure like sparsity, covariance estimation requires a number of samples of order $O(\ln p)$ \cite{rothman2008sparse}.

While estimating the covariance matrix or partial correlation matrix is challenging in ultra-high dimensions, it has been demonstrated in recent work that it is possible to accurately test the number of highly (partial) correlated variables under a false positive probability; in particular the probability that a variable is highly (partially) correlated with at least one other variable \cite{hero2011large,hero2012hub}. In \cite{hero2011large}, the ultra-high dimensional correlation screening problem is studied under a row-sparse assumption on the population covariance matrix. A phase transition in the number of false positive correlations was mathematically characterized as a function of the correlation threshold and the true covariance. In the case of block sparse covariance, the critical phase transition threshold becomes independent of the true covariance. While correlation screening finds the variables that have high marginal correlation with at least one other variable, partial correlation screening cares about the variables that have high conditional correlations with one other variable conditioned on the rest. In \cite{hero2012hub} the partial correlation screening problem was studied, and similar phase transition results as in correlation screening \cite{hero2011large} were obtained under the block-sparse assumption on the population covariance matrix. The survey \cite{hero2015foundational} reviews the correlation and partial correlation screening problem.


Despite these important advances in correlation and partial correlation screening, the screening framework proposed in \cite{hero2011large, hero2012hub} has some serious methodological, theoretical and practical shortcomings. For instance, results for partial correlation imposes a highly restrictive block sparsity assumption on the the true underlying correlation matrix. The block sparsity in \cite{hero2012hub} assumes only a small group of the variables are allowed to have correlation within the blocks and no correlations with variables outside the block. This assumption is severely restrictive for most modern applications since it is possible for variables to have correlations within a group and also correlations with variables outside their respective groups. Furthermore, expressions for false probabilities in  \cite{hero2011large, hero2012hub} require estimating dependence functionals. Estimating such functionals lead to computationally prohibitive non-parametric estimation, rendering the screening methodology disconnected from the very setting it was designed for. 

In this paper we propose a novel unifying framework for correlation and partial correlation screening that delivers a practical and scalable methodology in the ultra-high dimensional regime, which is simultaneously armed with theoretical safeguards. We derive results for the mean number of highly correlated or partial correlated variables, and quantify the discovery rate in \cite{hero2012hub} by relaxing block-sparse assumption to a weaker $(\tau,\kappa)$ sparsity assumption, defined in Section \ref{sec:taukappaspa}, on the population covariance matrix. The block-sparse assumption is a special case of the $(\tau,\kappa)$ sparsity assumption. Resulting approximations under this generalized covariance structure $(\tau,\kappa)$  also do not depend on dependence measures/functionals. Moreover, new results on the variance of the number of highly correlated or partial correlated variables are obtained in this paper, which in turn provide more information on the distribution (tail probability for instance) of the number of highly correlated or partial correlated variables, and provide a nontrivial bound on the discovery rate by second moment method. The results in this paper holds for both correlation and partial correlation screening. We show that the approximations of the mean and variance of the number of highly correlated variables, and false discovery probabilities, are the same as those quantities for partial correlation screening. This important duality naturally stems from new results relating the the score representation for correlation screening to that of partial correlation screening. The proofs of the generalized results in this paper are self-contained and are based on concentration of random matrices.  

The remainder of this paper is organized as follows. We begin in Section \ref{Hubfra} by giving the framework. In Section \ref{sec:asspre} assumptions and preliminaries are presented. Section \ref{mainres} is devoted to the statement of our main result and discussion of its consequences. Section \ref{simulation} provide some numerical simulations to verify our results. Subsequent sections are devoted to proofs of the main results, including a key observation, the almost distance preserving property between $\Yma$-score for partial correlation screening and $\Uma$-score for correlation screening (Section \ref{sec:distancepreserving}), and new results on Random Matrix with columns distributed \emph {i.i.d} uniformly on the sphere (Section \ref{ranmatunisph}). A number of technical proofs and auxiliary results are given in the Appendix.





\section{Introduction\YW{Old Version by Yun}} 
In this paper we consider the problem of screening $\nn$ independent and identically distributed $p$-variate samples for variables that have high correlation or partial correlation with at least one other variable in the ultra-high dimension regime $\nn \leq C_0\ln p$.\footnote{Here $C_0$ is some universal constant satisfying $C_0\geq 1$. Universal constant, or absolute constant, is a constant that doesn't depend on any parameter.} In the screening one applies a threshold to  sample correlation matrix or the sample partial correlation matrix to detect variables with at least one significant correlation. 

This problem of ultra dimension is important since in many applications the per-sample cost of collecting high dimensional data is much more costly than per-variable cost! For example, in biotech the cost of high throughput technology, like oligonucleotide gene microchips and RNAseq assays is decreasing, while the cost of biological samples isn't decreasing at the same rate \cite{hero201615}. In such a situation $p$ is much larger than $\nn$.

The ultra-high dimension regime $\nn\leq C_0\ln p$ is very challenging since the number of  samples is insufficient to apply many (if not most) reliable statistical methods. For example, one way to do the screening is firstly estimate the population covariance matrix, from which one estimates the inverse covariance, which is a proper estimation to the partial correlation matrix. However, to get a reliable estimate for general covariance matrix, the number of samples $\nn$ must be at least $O(p)$ as shown in Section 5.4.3. in \cite{vershynin2012introduction}. Even if the covariance matrix has special structure like sparsity, the covariance estimation requires a number of samples of order $O(\ln p)$ \cite{rothman2008sparse}.

While estimating the covariance matrix or partial correlation matrix is challenging in ultra-high dimension, it is possible to accurately test the number of highly (partial) correlated variables under a false positive probability; specially and the probability of at least one highly (partial) correlated variable \cite{HerRajlar, HerRajhub}. In \cite{hero2011large}, the ultra-high dimensional correlation screening problem is studied under a row-sparse assumption on the population covariance matrix. A phase transition in the number of false positive correlations was mathematically characterized as a function of the correlation threshold and the true covariance. In the case of block sparse covariance, the critical phase transition threshold becomes independent of the true covariance. While correlation screening finds the variables that have high marginal correlation with at least one other variable, partial correlation screening cares about the variables that have high conditional correlations with one other variable conditioned on the rest. In \cite{hero2012hub} the partial correlation screening problem was studied, and similar phase transition results as in correlation screening \cite{hero2011large} was obtained under the block-sparse assumption on the population covariance matrix. The survey \cite{hero2015foundational} reviews the correlation and partial correlation screening problem.

This paper extends the results of mean number of highly correlated or partial correlated variables and the discovery rate in \cite{hero2012hub} by relaxing block-sparse assumption to a weaker $(\tau,\kappa)$ sparsity assumption, defined in Section \ref{sec:taukappaspa}, on the population covariance matrix. The block sparsity in \cite{hero2012hub} assumes only a small group of the variables are allowed to have correlation within the groups, and hence is restrictive since it's possible variables has both correlations within the group and correlations with a few variables outside the groups. The $(\tau,\kappa)$ sparsity assumption take those cases into consideration, and reduces to the block-sparse assumption as a special case. Moreover, an new result on approximation of the variance of number of highly correlated or partial correlated variables are obtained in this paper, which provide more information on the distribution (tail probability for instance) of the number of highly correlated or partial correlated variables, and provide a nontrivial bound on the discovery rate by second moment method. 

The results in this paper holds for both correlation and partial correlation screening. We show that the approximations of mean, variance of number of highly correlated variables, and the probability that there exists some highly correlated pair are the same as those quantities for partial correlation screening. This fact come from the scores representation for correlation and partial correlation are almost the same. However, the results for partial correlation screening require the ultra dimensionality while it's not essential for correlation screening. 

The remainder of this paper is organized as follows. We begin in Section \ref{Hubfra} by giving the framework. In Section \ref{sec:asspre} assumptions and preliminaries are presented. Section \ref{mainres} is devoted to the statement of our main result and discussion of its consequences. Section \ref{simulation} provide some numerical simulations to verify our results. Subsequent sections are devoted to proofs of the main results, including a key observation, the almost distance preserving property between $\Yma$-score for partial correlation screening and $\Uma$-score for correlation screening (Section \ref{sec:distancepreserving}), and new results on Random Matrix with columns distributed i.i.d. uniformly on the sphere (Section \ref{ranmatunisph}). A number of technical proofs and auxiliary results are given in the Appendix.

==> sections/redudant_prelim.tex <==
%\section{Geometric Interpretation}
%\label{sec:asspre}

%\subsection{Multivariate normal representation}
%\label{sec:reduction}

%Theorem \ref{cor:Poissonlimit} establishes that the sequence of each of the $6$ random quantities $\{N_i^{(k)}: k\in \{\Rma,\Pma\}, i\in \{E_\delta, \breve{V}_\delta, V_\delta \} \}$, converges in distribution to a compound Poisson random variable, of which the increment has distribution $\bm{\zeta}_{n,\delta}$ defined in \eqref{eqn:incrementsizelimitdef}. Note $\bm{\zeta}_{n,\delta}$ is defined in terms of $\alpha_\ell$, the probability that there are exactly $\ell-1$ vertices of maximum degree $\delta-1$ in a random geometric graph. \mypurple{In this section we constructed random geometric graphs that are equivalent to empirical correlation graph and empirical partial correlation graph such that the geometric content in the increment of the limit Compound Poisson become more transparent.}

\subsection{Score representations of sample correlation and partial correlation}
\label{sec:scorerep}

In this subsection, the $\Uma$-score and the $\Yma$-score respectively for the sample correlation and the sample partial correlation  are defined. These scores will serve as the vertices set on which the random geometric graphs are constructed in Subsection \ref{sec:rangeo}. We first present two useful canonical representations \myred{of} our model. 

\myred{The first representation is to represent functions of $\Rma$ for $\Xma$ from a vector elliptically contoured distribution $\mathcal{VE}(\bm{\mu},\Sigmama,g)$ as functions of $\Rma$ for $\Xma$ from a centered matrix normal distribution $\mathcal{VE}(\bm{0},\Sigmama,g_0)$. }  
%\noindent 
%{\bf \YW{Representation as from centered matrix normal data} } \\
%\noindent 
The following lemma is an immediate result of the theorem in Section 6 of \cite{anderson1992nonnormal}.
\begin{lem} \label{prop:anderinv}
    Suppose $\Xma \sim \mathcal{VE}(\muve,\Sigmama,g)$. Then the distribution of $\Rma$ defined in \eqref{defR} is invariant to $g$ and $\muve$.
\end{lem}

Since the quantities of interest in this paper are  $\bar{N}_\delta$, functions of $\Rma$, their distribution are also invariant to $g$ and $\muve$ when $\Xma \sim \mathcal{VE}(\muve,\Sigmama,g)$. Specifically, we may choose $ g(w)=g_0(w)=(2\pi)^{-\frac{\nn p}{2}}\exp(-\frac{1}{2}w)$ and $\muve = \bm{0}$ such that $\Xma$ follows the centered matrix normal distribution $\mathcal{VE}(\bm{0},\Sigmama,g_0)$. That is, $\{\xve^{(i)}\}_{i=1}^{\nn}$, the rows of $\Xma$, can be taken as i.i.d. samples from $\Nc(\bm{0},\Sigmama)$, without changing the distribution of $\bar{N}_\delta$. \myred{Thus for the rest of the paper $\Xma \sim \mathcal{VE}(\muve,\Sigmama,g)$ implicitly means $\mathcal{VE}(\bm{0},\Sigmama,g_0)$ by Lemma \ref{prop:anderinv} and hence we suppose $\Xma$ follows the centered matrix normal distribution $\mathcal{VE}(\bm{0},\Sigmama,g_0)$. As a consequence, $\Sigma_{ij}=0$ implies variable $i$ and variable $j$ are independent.} In particular, the different sparsity conditions discussed in Subsection \ref{sec:taukappaspa} imposed on $\Sigmama$ induces different independence structures between variables in the model. %, which is explored in Subsection \ref{sec:taukappaspa}.


The second representation represents the sample covariance matrix defined in \eqref{def:samcov} by a sample second moment of the projected data. %\noindent 
%{\bf Representation of sample covariance matrix by sample second moment} \\
It is shown in Theorem 3.3.2 \cite{anderson2003introduction} that the sample covariance matrix of $\nn$ i.i.d. normal random vector can be represented as the sample second moment of $\nn-1$ i.i.d. zero-mean normal random vectors. Specifically, define
the orthogonal $\nn \times \nn$ matrix $\Hma = [\nn^{-\frac{1}{2}}\bm{1}, \Hma_{2:\nn}]^T$. The matrix $\Hma_{2:\nn}$ can be obtained by
Gramm-Schmidt orthogonalization and satisfies the properties
$$
\bm{1}^T\Hma_{2:\nn} = \bm{0}, \quad \Hma_{2:\nn}^T\Hma_{2:\nn} = \Ima_{\nn - 1}.
$$
Then 
\begin{equation}
\tilde{\Xma} = \Hma_{2:\nn} \Xma \in \R ^{(\nn-1) \times p} \label{eqn:Xtildef}
\end{equation}
has i.i.d. rows $\{\tilde{\xve}^{(i)}\}_{i=1}^{\nn-1}$ drawn from $\Nc(\bm{0},\Sigmama)$. Moreover the sample covariance matrix defined in \eqref{def:samcov}
\begin{equation}
\Sma = \frac{1}{\nn-1}\Sum_{i=1}^{\nn-1}\tilde{\xve}^{(i)}(\tilde{\xve}^{(i)})^T=\frac{1}{\nn-1}\tilde{\Xma}^T\tilde{\Xma}. \label{eqn:sigdef}
\end{equation}
That is, the sample covariance matrix of the data matrix $\Xma$, defined in \eqref{def:samcov}, is the same as the sample second moment of the data matrix $\tilde{\Xma}$. It follows that $\Sigma_{ij}=0$ implies $\tilde{\xve}^{(i)}$ is independent of $\tilde{\xve}^{(j)}$.\\


\mypurple{ We now proceed to define and analyze the scores representation of $\Rma$ and $\Pma$. From the second representation above,}
$\{\tilde{\xve}^{(i)}\}_{i=1}^{\nn-1}\subset \R^p$, the rows of $\tilde{\Xma}$, are i.i.d. copy from $\Nc(\bm{0},\Sigmama)$. Let $\{\tilde{\xve}_i\}_{i=1}^{p}$ denote the columns of $\tilde{\Xma}$. Then $\uve_i\vcentcolon=\frac{\tilde{\xve}_i}{\|\tilde{\xve}_i\|_2}\in \R^{\nn-1}$ has distribution $\unif(S^{\nn-2})$ since $\tilde{\xve}_i$ contains $n-1$ i.i.d. normal coordinates, where $\|\cdot\|_2$ for a vector represents its Euclidean distance to the origin. Denote
$$
\Uma = [\uve_1, \uve_2, \ldots, \uve_p] \in \R^{(\nn -1) \times p}
$$
and it follows from \eqref{eqn:sigdef} and \eqref{defR} that
\begin{equation}
\Rma= \Uma^T\Uma.  \label{Rfac}
\end{equation}
The $\Uma$ in equation \eqref{Rfac} is referred to as $\Uma$-score of the sample correlation matrix \cite{hero2011large, hero2012hub}. Note our formulation of $\Uma$-score is slightly different from the formulation in \cite{hero2011large, hero2012hub}, but it's an easy task to check the two different formulations are equivalent. \YW{Moreover, it follows that $\uve_i$ and $\uve_j$ are independent provided the population covariance $\Sigma_{ij}=0$. }

The normalized outer product of $\Uma$, defined by 
\begin{equation}
\Bma =\frac{\nn-1}{p}\Uma\Uma^T\in \R^{(\nn-1)\times (\nn-1)} \label{eqn:Bdef}
\end{equation}
 will play an important role in the analysis of empirical partial correlation graph. 
\begin{lem}
\label{lem:Binv}
Let $\Xma \sim \mathcal{VE}(\muve,\Sigmama,g)$ and $p\geq n$. Then $\Bma$ is invertible with probability $1$.
\end{lem}

By Lemma 1 in \cite{hero2012hub}, provided $\Uma\Uma^T$ is invertible or, equivalently, $\Bma$ is invertible, \myred{the Moore-Penrose pseudo-inverse of $\Rma$ can be expressed as follows:}
\begin{equation}
\label{Rdagdef}
\Rma^\dagger = \Uma^T[\Uma\Uma^T]^{-2}\Uma=\left(\frac{p}{\nn-1}\right)^2\Uma^T\Bma^{-2}\Uma.
\end{equation}
 It follows from Lemma \ref{lem:Binv} that equation \eqref{Rdagdef} holds $a.s.$. Define $\Ama=\Bma^{-1}$ , $\bar{\Yma}=\Ama\Uma$ and hence
\begin{equation}
\label{RdagYbar}
\Rma^\dagger = \left(\frac{p}{\nn-1}\right)^2 \bar{\Yma}^T\bar{\Yma} \quad a.s. .
\end{equation}
Further define
\begin{align*}
\yve_i &= \bar{\yve}_i/\|\bar{\yve}_i\|_2, \quad \forall\ i\in p, \\
\Yma & = [\yve_1,\yve_2,\ldots,\yve_p]\in \R^{(\nn-1)\times p},
\end{align*}
and thus
\begin{equation}
\Pma = \Yma^T\Yma \quad a.s.  \label{Pfac}
\end{equation}
by equation \eqref{Pdef} and \eqref{RdagYbar}. $\Yma$ in equation \eqref{Pfac} is referred to as the $\Yma$-score representations of the sample partial correlation matrix \cite{hero2012hub}. Similar to the $\Uma$-score, one can easily verify that our formulation of $\Yma$-score is equivalent to that in \cite{hero2012hub}.

Let $\sigma^{n-2}$ be the spherical measure on $S^{n-2}$, i.e. $\sigma^{n-2}$ is the probability measure corresponding to the uniform distribution on $S^{n-2}$. Denote by $f_{\uve_{j_1},\uve_{j_2},\cdots,\uve_{j_m}}$ the joint density of $j_1$-th, $j_2$-th, $\ldots$, $j_m$-th column of $\Uma$ with respect to the product measure $\otimes^m \sigma^{n-2} := \underbrace{\sigma^{n-2}\otimes \sigma^{n-2} \otimes \cdots \otimes \sigma^{n-2}}_{m}$. The next lemma establishes that $f_{\uve_{j_1},\uve_{j_2},\cdots,\uve_{j_m}}$ is bounded by $\mu_{n,m}(\Sigmama)$. \myred{This highlights the role of $\mu_{n,m} (\Sigmama)$ since the distribution of the three quantities $N_{\VVV_\delta}^{(\Rma)}$ ,$N_{\VV_\delta}^{(\Rma)}$, $\Nedged^{(\Rma)}$, as discussed in Subsection \ref{sec:upperboundjointdensity}, have a local property in the sense that their distribution depends only on the joint density of $f_{\uve_{j_1},\uve_{j_2},\cdots,\uve_{j_m}}$ for every possible collection of $\{j_i\}_{i=1}^m$ and some constant $m=2\delta+2$.}

\begin{lem} \label{lem:densitybou}
    Let $\Xma\sim \mathcal{VE}(\bm{\mu}, \Sigmama, g)$. Consider a set of distinct indexes $\mathcal{J}=\{j_i: 1\leq i \leq m\}\subset [p]$.
    \begin{enumerate}[label=(\alph*)]        
        \item \label{item:densityboua}
        $$
        \mu_{n,m}(\Sigmama_{\mathcal{J}}) \leq \mu_{n,m} (\Sigmama)
        $$
        
        \item \label{item:densityboub}  
        The joint density of any subset of $m$ columns of $\bm{U}$-score w.r.t. $\otimes^m \sigma^{n-1}$ is upper bounded by $\mu_{n,m} (\Sigmama)$:
        $$f_{\uve_{j_1},\uve_{j_2},\cdots,\uve_{j_m}}(\vve_1,\vve_2,\cdots,\vve_m)  \leq \mu_{n,m}(\Sigmama_{\mathcal{J}}) \leq \mu_{n,m} (\Sigmama),  \quad \forall \  \vve_i\in S^{n-2}, \forall\ i\in [m]. $$
         Here $\mu_{n,m}(\Sigmama_{\mathcal{J}})$ is well defined since $\mu_{n,m}(\cdot)$ is invariant to simultaneously applying a permutation to both rows and columns.
        \item \label{item:densitybouc}
        Let $h:\left(S^{n-2}\right)^m\to \R$ be a nonnegative Borel measurable function. Then 
        \[
        \E h(\uve_{j_1},\uve_{j_2},\cdots,\uve_{j_m})\leq \mu_{n,m} (\Sigmama_{\mathcal{J}}) \E h(\uve_{j_1}',\uve_{j_2}',\cdots,\uve_{j_m}')\leq \mu_{n,m} (\Sigmama) \E h(\uve_{j_1}',\uve_{j_2}',\cdots,\uve_{j_m}'),    
        \]
        where $\{\uve_{j_\ell}'\}_{\ell=1}^m$ are i.i.d. distributed as \unif$(S^{n-2})$.
    \end{enumerate}
\end{lem}

\begin{rem}
    In Lemma \ref{lem:densitybou} \ref{item:densityboua}, since $\Sigmama_{\mathcal{J}}$ is an $m$ by $m$ symmetric positive definite matrix, by the definition in \eqref{eqn:munmA}, $$\mu_{n,m}(\Sigmama_{\mathcal{J}})=\begin{cases} [\mu(\Sigmama_{\mathcal{J}})]^{-\frac{n-1}{2}}, &  \Sigmama_{\mathcal{J}} \text{ not diagonal, }  \\
    1, & \Sigmama_{\mathcal{J}} \text{  diagonal. }
     \end{cases}$$
     \myeoe
\end{rem}

The proof of Lemma \ref{lem:densitybou} \ref{item:densityboub} is deferred to Appendix \ref{sec:proofdensitybou}. Part \ref{item:densitybouc} immediately follows from part \ref{item:densityboub} by writing expectation as integrals. Part \ref{item:densityboua} follows trivially from $\mu_m(\Sigmama_{\mathcal{J}})=\mu(\Sigmama_{\mathcal{J}})\geq \mu_m(\Sigmama)$.

Lemma \ref{lem:densitybou} \ref{item:densitybouc} is useful since when calculating expectation of nonnegative function of any $m$ columns of $\Uma$, one may always assume the associated columns $\{\uve_j\}$ are independent $\unif(S^{n-1})$ \YW{up to} an additional multiplicative factor $\mu_{n,m}(\Sigmama)$.









\subsection{Random pseudo geometric graphs}
\label{sec:rangeo}

\mypurple{
In this subsection we define random pseudo geometric graphs and provide an equivalent formulation of our model, of which the vertex sets are the $\Uma$ and $\Yma$ scores defined in Subsection \ref{sec:scorerep}. We also define the increment distribution of the compound Poisson that non-asymptotically approximates the $\bar{N}_\delta$.
}

From equation \eqref{Rfac} and the fact that columns of $\Uma$ have Euclidean norm $1$,
\begin{equation}
R_{ij}=\uve_i^T\uve_j=1- \frac{\|\uve_i-\uve_j\|_2^2}{2} =  \frac{\|\uve_i+\uve_j\|_2^2}{2} -1. \label{eqn:cortoycol}
\end{equation}
For a threshold $\rho\in [0,1)$, define $r_\rho:=\sqrt{2(1-\rho)} \in (0,\sqrt{2}]$. By equation \eqref{eqn:cortoycol},
$$
\{R_{ij} \geq \rho\} =\{\| \uve_i-\uve_j\|_2\leq \sqrt{2(1-\rho)} \}=\{ \|\uve_i-\uve_j\|_2 \leq r_\rho\}.
$$
and similarly,
$$
\{R_{ij} \leq -\rho\} =  \{ \|\uve_i+\uve_j\|_2 \leq r_\rho\}.
$$
The two preceding expressions yield
\begin{equation}
 \{ |R_{ij}| \geq \rho \} = \{\|\uve_i+\uve_j\|_2 \leq r_\rho\}\cup \{\|\uve_i-\uve_j\|_2 \leq r_\rho\}.   
\label{eqn:corphiequzer}
\end{equation}
An analogous derivation yields the following for the empirical partial correlation graph,
\begin{equation}
 \{ |P_{ij}| \geq \rho \} = \{\|\yve_i+\yve_j\|_2 \leq r_\rho\}\cup \{\|\yve_i-\yve_j\|_2 \leq r_\rho\}.   \label{phiequzer}
\end{equation}
Based on \eqref{eqn:corphiequzer} and \eqref{phiequzer}, first presented in \cite{hero2011large,hero2012hub}, we now introduce some novel geometry connecting to random geometric graphs. Note \eqref{eqn:corphiequzer} indicates, $\{|R_{ij}|\geq \rho\}$, the event when sample correlation between $i$-th and $j$-th variables exceed the threshold $\rho$, or equivalently, the event when there exists a edge connecting the $i$-th and $j$-th vertices in the empirical correlation graphs $\Gc_{\rho}(\Psima^{(\Rma)})$, is the same as the event that $\uve_i$ and $\uve_j$, the associated $\Uma$-score, lie in some geometric set on $S^{\nn-2}\times S^{\nn-2}$. This insight provides an equivalent way to construct $\Gc_{\rho}(\Psima^{(\Rma)})$ through the $\Uma$-scores and similar interpretation can be drawn for \eqref{phiequzer}. Such equivalent construction is made formal in the next few paragraphs.

\begin{comment}
Recall given a set of points $\{ \vve_i  \}_{i=1}^m$ in $\R^{\mathscr{N}}$, denote by $\textbf{Ge}\left(\{\vve_i  \}_{i=1}^{m}, r  ; m, \mathscr{N} \right)$ the geometric graph\index{geometric graph} with radius $r$, defined as follows. The vertex set of the graph is $\{ \vve_i  \}_{i=1}^m$, and there is an edge between $\vve_i$ and $\vve_j$ if $\|\vve_i-\vve_j\|_2 \leq r$.
Next, define a similar but different geometric graph, which is closely related to the empirical correlation and partial correlation graphs. 
\end{comment}

\begin{definition}[Pseudo geometric graph\index{pseudo geometric graph}]
    \label{def:pge}
    Given $m\geq 2$ and a set of points $\{ \vve_i  \}_{i=1}^m$ in $\R^{\mathscr{N}}$, denote by $\textbf{PGe}\left(\{\vve_i  \}_{i=1}^m, r  ; m, \mathscr{N} \right)$ the pseudo geometric graph with radius $r$, defined as follows. The vertex set of the graph is $\{ \vve_i  \}_{i=1}^m$, and there is an edge between $\vve_i$ and $\vve_j$ if $\textbf{dist}(\vve_i,\vve_j):= \min\left\{\|\vve_i-\vve_j\|_2,\|\vve_i+\vve_j\|_2 \right \}  \leq r$.
\end{definition}
It's easy to verify that $\textbf{dist}(\cdot,\cdot)$ has the following properties: for $\forall \vve_1,\vve_2,\vve_3\in \R^m$,
\begin{enumerate}
\item     $\textbf{dist}(\vve_1,\vve_2)\geq 0$;
\item   $\textbf{dist}(\vve_1,\vve_2) = 0$ if only if $\vve_1 = \vve_2$ or $\vve_1 = - \vve_2$;
\item   $\textbf{dist}(\vve_1,\vve_2) = \textbf{dist}(\vve_2,\vve_1)$ and $\textbf{dist}(\vve_1,\vve_2) = \textbf{dist}(\vve_1,-\vve_2)$
\item $\textbf{dist}(\vve_1,\vve_2)\leq \textbf{dist}(\vve_1,\vve_3) + \textbf{dist}(\vve_3,\vve_2)$.
\end{enumerate}
That is, $\textbf{dist}(\cdot,\cdot)$ is a pseudo metric on $\R^\mathscr{N}$, which explains the name pseudo geometric graph in Definition \ref{def:pge}. Also, $\textbf{dist}(\cdot,\cdot)$ is indeed a metric on the quotient space of $\R^\mathscr{N}$ with any two points symmetric about origin identified. 

If the set of points generating geometric graphs or pseudo geometric graphs are random, then the corresponding graphs are called random geometric graphs or random pseudo geometric graphs. 

%Recall in the empirical correlation graph, there is an edge between vertices $i$ and $j$ if their corresponding sample correlation $|R_{ij}|\geq \rho$, which is equivalent to $\textbf{dist}(\uve_i,\uve_j)\leq r_\rho$ by \eqref{eqn:corphiequzer}. 
With the above definitions and by the discussions preceding Definition \ref{def:pge}, the empirical correlation graph $\Gc_{\rho}(\Psima^{(\Rma)})$ is isomorphic to $\textbf{PGe}\left(\{\uve_i  \}_{i=1}^p, r_\rho  ; p, n-1 \right)$, the random pseudo geometric graph generated by $\Uma$-scores. Even though $\textbf{PGe}\left(\{\uve_i  \}_{i=1}^p, r_\rho  ; p, n-1 \right)$ has additional geometric contents since each vertex in it is a specific point in $S^{n-2}$, it's not necessary to differentiate it from the empirical correlation graph as long as only the graph properties are of concerned. As an example, we may refer to $N_{V_\delta}^{(\Rma)}$ the number of vertices with degree at least $\delta$ in $\textbf{PGe}\left(\{\uve_i  \}_{i=1}^p, r_\rho  ; p, n-1 \right)$ as well. An entirely analogous analysis applies to empirical partial correlation graph and  $\textbf{PGe}\left(\{\yve_i  \}_{i=1}^p, r_\rho  ; p, n-1 \right)$. This equivalent construction indicates that the distribution of each of the 3 quantities $\{N_{E_\delta}^{(k)},N_{\breve{V}_\delta}^{(k)},N_{V_\delta}^{(k)}  \}$ with $k=\Rma$ ($k=\Pma$) depends only on the pairwise pseudo distances $\textbf{dist}(\cdot,\cdot)$ between columns of $\Uma$ ($\Yma$). 

%In Subsection \ref{sec:rangeo} we represent the empirical correlation graph as random pseudo geometric graph with $\Uma$-scores $\{\uve_i\}_{i=1}^p$ as vertices. 
\myred{
The random pseudo geometric graphs analyzed above bear some similarities to the random geometric graphs in \cite{penrose2003random}. %From the previous paragraph, $N_{E_\delta}^{(\Rma)}$ is the star subgraph counts and $N_{V_\delta}^{(\Rma)}$ is the number of vertices of degree at least $\delta$ of the random pseudo geometric graph $\textbf{PGe}\left(\{\uve_i  \}_{i=1}^p, r_\rho  ; p, n-1 \right)$. 
In particular, the monograph \cite{penrose2003random} studies the number of \emph{induced} subgraphs isomorphic to a given graph, typical vertex degrees, and other graphical quantities of random geometric graphs. The difference between the random pseudo geometric graphs in this paper and the random geometric graphs in \cite{penrose2003random} is that our vertices $\uve_i$ lie on the unit sphere instead of the whole Euclidean space and our distance is $\textbf{dist}(\cdot,\cdot)$ instead of Euclidean distance. Another key difference is that no independence among all vertices $\uve_i$ are imposed in our model. Indeed in our model, the correlations between vertices $\uve_i$ are encoded by a sparse matrix $\Sigmama$, where \cite{penrose2003random} impose the strong assumption that vertices of the random geometric graph are i.i.d.. In \cite{penrose2003random} an example concerning asymptotic compound Poisson limit for the number of vertices with degree at least $3$ was presented (cf. the Example after Corollary 3.6).
%The asymptotic compound Poisson limit for the number of vertices of degree at least $3$ is intuitively discussed in the Example after Corollary 3.6 in \cite{penrose2003random}, without characterizing the parameters of the compound Poisson. Here in Theorem \ref{cor:Poissonlimit}, %and Theorem \ref{thm:Poissonultrahigh}, 
%we prove the asymptotic compound Poisson limit and characterizes the parameters of the limit.
}

\begin{comment}
The differences between our model and the random geometric model are 1) our vertices $\uve_i$ lie in the unit sphere instead of the whole Euclidean space; 2) the distance is $\textbf{dist}(\cdot,\cdot)$ instead of Euclidean distance; 3) no independence among all vertices $\uve_i$ are imposed. Instead, their correlations are encoded by a sparse $\Sigmama$.
\end{comment}

Recall $\nmd\left(\{\vve_i  \}_{i=1}^m, r  ; m, \mathscr{N} \right)$ denotes the number of vertices of degree $m-1$ in the geometric graph $\textbf{Ge}\left(\{\vve_i  \}_{i=1}^m, r  ; m, \mathscr{N} \right)$. When $m\geq 3$, $\nmd\left(\{\vve_i  \}_{i=1}^m, r  ; m, \mathscr{N} \right)$ is also the number of subgraphs of $\textbf{Ge}\left(\{\vve_i  \}_{i=1}^m, r  ; m, \mathscr{N} \right)$ isomorphic to $\Gamma_{m-1}$. Define $\pnmd\left(\{\vve_i  \}_{i=1}^m, r  ; m, \mathscr{N} \right)$ analogously for pseudo geometric graph.   



Denote by $\text{deg}(\cdot)$ the degree of a given vertex in the graph. Consider $\{\uve'_i\}_{i=1}^{\delta+1}\ \overset{\text{i.i.d.}}{\sim} \ \text{unif}(S^{n-2})$. Denote the conditional probability that there are $\ell$ vertices of degree $\delta$ in $\pnmd\left(\{\uve'_i  \}_{i=1}^{\delta+1}, r_\rho  ; \delta+1, n-1 \right)$ by
\begin{equation}
\alpha_{n,\delta}(\ell,r_\rho) := \P\left(\pnmd\left(\{\uve'_i  \}_{i=1}^{\delta+1}, r_\rho ; \delta+1, n-1 \right)=\ell|\text{deg}(\uve'_1)=\delta\right),\quad \forall \ell\in [\delta+1]. \label{eqn:alphandeltarho}
\end{equation} 
$\alpha_{n,\delta}(\ell,r_\rho)$ depends only on $n$, $\delta$ and the threshold $\rho$ and is abbreviated as $\alpha(\ell,r_\rho)$ when there is no confusion.  Moreover, $\alpha(\ell,r_\rho)=0$ when $\ell \geq \delta+2$. Define a probability  distribution $\bm{\zeta}_{n,\delta,\rho}$ supported on $[\delta+1]$ with
\begin{equation}
\bm{\zeta}_{n,\delta,\rho}(\ell) = \frac{\alpha(\ell,r_\rho)/\ell}{ \sum_{\ell=1}^{\delta+1} \left(\alpha(\ell,r_\rho)/\ell \right) }.  \label{eqn:zetandelrhodef}
\end{equation}


It will be shown in the next three subsections that the probability distribution $\bm{\zeta}_{n,\delta,\rho}$ is the distribution of the increment of the compound Poisson that non-asymptotically approximates the $\mathscr{L}(\bar{N_\delta})$. %It will also be shown by Lemma \ref{prop:rangeolimit}  $\bm{\zeta}_{n,\delta,\rho}(\ell)\to \bm{\zeta}_{n,\delta}(\ell)$ when $r_\rho\to 0$ or $\rho\to 1$.



==> sections/redudant_todolist.tex <==
\section{Things To be done}
\begin{enumerate}
	\item Simulation \YW{completed}
	    \begin{enumerate}
	    	\item Validate the number of discovery for small sample is a compound Poisson but not a Poisson; this includes the corner cases $N=4,\delta=2$; and a family of curves for different $\delta$; and a graph of total variation between samples to the compound poisson (need to add a divergence to Poisson as a comparison); and a graph for $\delta=1$ to see the convergence rate for different $\delta$;
	    	\item Comparison between result under different sparsity conditions on theorectical covariance matrix: $(\tau,\kappa)$ sparsity vs block sparsity vs diagonal matrix; vary the different sparsity level and see if there is a consequences
	    	\item Use the result to test the sparsity structure of the theorectical covariance matrix in the hypothesis testing-> test on different dense matrix and see  how the convergence behaves; vary the magnitude in a given type of dense matrix;  
	    	\item (might not be necessary for this paper) apply the result to some real data. Consider the familywise rate as in the hub screening paper. 
	    	\item (might not be necessary for this paper) closed form to approximate the phase transition for the compound Poisson result. or MCMC?
	    \end{enumerate}
	\item Organize the paper \YW{we are here}
	\item Introduction (look for possible new papers in the literature)
\end{enumerate}
